A Polar Code Based TIN-SIC Scheme for the Unsourced Random Access in the Quasi-Static Fading MAC

We consider a problem of unsourced random access in the quasi-static Rayleigh fading channel. In the previous work, the authors have proposed LDPC code based solutions based on joint and treat interference as noise in combination with successive interference cancellation (TIN-SIC) decoder architectures. The authors showed that TIN-SIC decoding significantly outperforms the joint decoding approach and much simpler from the implementation point of view. In this paper, we continue the analysis of TIN-SIC decoding. We derive a finite length achievability bound for TIN-SIC decoder using random coding and propose a practical polar code based TIN-SIC scheme. The latter's performance becomes significantly better in comparison to LDPC code based solutions and close to the finite length achievability bound.

==> tikz/color_scheme.tex <==
\def\PgfColorA{0, 0, 0}
\def\PgfColorB{27,158,119}
\def\PgfColorC{217,95,2}
\def\PgfColorD{117,112,179}
\def\PgfColorE{231,41,138}
\def\PgfColorF{102,166,30}
\def\PgfColorG{230,171,2}
\def\PgfColorH{166,118,29}

\definecolor{MainColorA}{RGB}{\PgfColorA}
\definecolor{MainColorB}{RGB}{\PgfColorB}
\definecolor{MainColorC}{RGB}{\PgfColorC}
\definecolor{MainColorD}{RGB}{\PgfColorD}
\definecolor{MainColorE}{RGB}{\PgfColorE}
\definecolor{MainColorF}{RGB}{\PgfColorF}
\definecolor{MainColorG}{RGB}{\PgfColorG}
\definecolor{MainColorH}{RGB}{\PgfColorH}

\def\colorA{MainColorA!100}
\def\colorB{MainColorB!100}
\def\colorC{MainColorC!100}
\def\colorD{MainColorD!100}
\def\colorE{MainColorE!100}
\def\colorF{MainColorF!100}
\def\colorG{MainColorG!100}
\def\colorH{MainColorH!100}
